Dialogizer: Context-aware Conversational-QA Dataset Generation from Textual Sources

To address the data scarcity issue in Conversational question answering (ConvQA), a dialog inpainting method, which utilizes documents to generate ConvQA datasets, has been proposed. However, the original dialog inpainting model is trained solely on the dialog reconstruction task, resulting in the generation of questions with low contextual relevance due to insufficient learning of question-answer alignment. To overcome this limitation, we propose a novel framework called Dialogizer, which has the capability to automatically generate ConvQA datasets with high contextual relevance from textual sources. The framework incorporates two training tasks: question-answer matching (QAM) and topic-aware dialog generation (TDG). Moreover, re-ranking is conducted during the inference phase based on the contextual relevance of the generated questions. Using our framework, we produce four ConvQA datasets by utilizing documents from multiple domains as the primary source. Through automatic evaluation using diverse metrics, as well as human evaluation, we validate that our proposed framework exhibits the ability to generate datasets of higher quality compared to the baseline dialog inpainting model.

==> rsc/Table_case.tex <==
\begin{table*}[t]
\renewcommand{\arraystretch}{1.3}
\centering
\resizebox{0.95\textwidth}{!}{% 
\begin{tabular}{c|l|l|c|c}
\hline  \hline
\textbf{Model}    & \multicolumn{1}{c|}{\textbf{Generated Question}}                                                                & \multicolumn{1}{c|}{\textbf{Answer}}                                                                                                                                             & \textbf{Question Type} & \textbf{RQUGE} \\ \hline
\textbf{baseline} & \begin{tabular}[c]{@{}l@{}}What else did Daniel Offenbacher \\ do after playing football?\end{tabular}          & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}In January 2012 he went out on loan to Blau-\\ Wei\textbackslash{}u00df Linz in the First league (2nd Austrian League).\end{tabular}} & concept                & 3              \\ \cline{1-2} \cline{4-5} 
\textbf{ours}     & \textbf{\begin{tabular}[c]{@{}l@{}}What else did Daniel Offenbacher \\ do after playing football?\end{tabular}} &                                                                                                                                                                                  & concept                & 3              \\ \hline  \hline
\textbf{ours}     & \begin{tabular}[c]{@{}l@{}}What else did Daniel Offenbacher do\\ after playing football?\end{tabular}           & \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}In January 2012 he went out on loan to Blau-\\ Wei\textbackslash{}u00df Linz in the First league (2nd Austrian League).\end{tabular}} & concept                & 3              \\ \cline{1-2} \cline{4-5} 
\textbf{ours}     & \begin{tabular}[c]{@{}l@{}}What else did Daniel Offenbacher do \\ after playing football?\end{tabular}          &                                                                                                                                                                                  & concept                & 3              \\ \cline{1-2} \cline{4-5} 
\textbf{ours}     & \textbf{\begin{tabular}[c]{@{}l@{}}What else did Daniel Offenbacher \\ do after playing football?\end{tabular}} &                                                                                                                                                                                  & concept                & \textbf{3}     \\ \hline  \hline
\end{tabular}
}
\caption{Case Study}
\label{table_case}
\end{table*}


==> text/z2.Background.tex <==
%dialog inpainting strength
%Dialog Inpainting has highly valuable due to the abundance of high-quality documents authored by domain experts available online, and its capability to convert them into dialog datasets without any loss of information.
To overcome the data scarcity problem in ConvQA, an automatic ConvQA dataset generation framework called dialog inpainting has been proposed. Similar to filling in the other side of a phone call conversation by overhearing someone else's dialogue, this methodology utilizes sentences from text documents as one person's dialogue and generates the remaining dialogues to complete the conversation. The efficiency of dialog inpainting as a ConvQA dataset generation framework is supported by the ability to automatically transform any text data into a dialog format, as evidenced by the abundance of high-quality documents annotated by domain experts, such as Wikipedia or Pubmed. However, we have been experimentally observed that the questions generated by the standard dialog inpainter lack context relevance. %
% Training - Dialog Reconstruction
The dialog inpainter is exclusively trained with the Dialog Reconstruction task, which includes the random masking of one utterance $d_m(t)=(u_1,u_2,...,u_{t-1}, \bullet ,u_{t+1},...,u_T)$ in the dialogue $d=(u_1,u_2,...,u_t,...,u_T)$, with the masked utterance denoted by the symbol $\bullet$. The objective is to reconstruct the missing utterance $u_t$. 

%L_DR 식 추가

However, as depicted in Figure~\ref{fig_intro}, we note that the questions generated by the original dialog inpainter demonstrate suboptimal quality and a deficiency in contextual relevance. In this study, we propose Dialogizer, a framework that aims to address the limitations not covered by the dialog reconstruction task and allows for the generation of stable and contextually relevant ConvQA datasets.

% Inference <- autoregressively
\iffalse
\subsection{Inference}
The dialog inpainter transfroms the input document or passage to dialog. In a similar vein to the original dialog inpainter, the overall process and inference procedure remain analogous. During the inference stage, the dialog inpainter fills in the masked utterances in the partial dialog $(\bullet, s_1, \bullet, s_2, ..., \bullet, s_m)$ for a given document $(s_1, s_2, ..., s_m)$. To obtain a hint that the speaker needs to respond to a question, we append a prompt $s_{prompt}$ using the document title, resulting in $(s_{prompt}, \bullet, s_1, ..., s_m)$ for inpainting. Furthermore, to avoid discrepancies with the dialog reconstruction approach that generates one utterance at a time during training, we employ an autoregressive generation process.
\fi
